False Consensus, Information Theory, and Prediction Markets

We study a setting where Bayesian agents with a common prior have private information related to an event's outcome and sequentially make public announcements relating to their information. Our main result shows that when agents' private information is independent conditioning on the event's outcome whenever agents have similar beliefs about the outcome, their information is aggregated. That is, there is no false consensus. Our main result has a short proof based on a natural information theoretic framework. A key ingredient of the framework is the equivalence between the sign of the ``interaction information'' and a super/sub-additive property of the value of people's information. This provides an intuitive interpretation and an interesting application of the interaction information, which measures the amount of information shared by three random variables. We illustrate the power of this information theoretic framework by reproving two additional results within it: 1) that agents quickly agree when announcing (summaries of) beliefs in round robin fashion [Aaronson 2005]; and 2) results from [Chen et al 2010] on when prediction market agents should release information to maximize their payment. We also interpret the information theoretic framework and the above results in prediction markets by proving that the expected reward of revealing information is the conditional mutual information of the information revealed.

==> quick.tex <==

\begin{theorem}[Convergence rate]\label{thm:quick}
With at most $\frac{I(X_1,X_2,...;W)}{\epsilon}\leq \frac{H(W)}{\epsilon}$ rounds, the agreement protocol achieves $\epsilon$-MI consensus. 
\end{theorem}


\begin{proof}
%To show the expected time when every agent $\epsilon$-agrees with the outsider is bounded, we use a natural potential function which is the amount of information aggregated. 

Because mutual information is monotone, the amount of information aggregated $I(\Pi^t;W)$ is an increasing function with respect to $t$. Moreover, we will show that when a round does not achieve $\epsilon$-MI consensus, the expected amount of aggregated information increases by at least $\epsilon$.  

Formally, when a round $t$ does not achieve $\epsilon$-MI consensus, there exists an agent $i$ such that $I(X_i;W|\Pi_i^t)> \epsilon$. Thus, the expected amount of aggregated information increases by at least $\epsilon$ in round $t$ because\[ I(\Pi^t;W)-I(\Pi^{t-1};W)\geq I(\Pi_{i+1}^t;W)-I(\Pi_{i}^t;W)=I(\Pi_{i+1}^t;W|\Pi_{i}^t)= I(X_i;W|\Pi_i^t)> \epsilon \]

The first inequality holds because $I(\Pi^t;W)\geq I(\Pi_{i+1}^t$ and $I(\Pi^{t-1};W)\leq I(\Pi_{i}^t;W)$. That is, the amount of information increased in a single round $t$ must be greater than the amount of information increased in a single step in round $t$. The second equality holds due to chain rule and the fact that $\Pi_{i+1}^t$ contains $\Pi_{i}^t$. The third equality holds since agent $i$ will rationally updates her belief to $p_i^t$ where $\forall w, p_i^t(w)=\Pr[W=w|X_i,\Pi_{i}^t]$ and declares it. This declaration will be added to $\Pi_{i+1}^t=(\Pi_i^t,p_i^t)$. 

Finally,because for all $t$, $I(\Pi^t;W)\leq I(X_1,X_2,...;W)\leq H(W)$, with at most $\frac{I(X_1,X_2,...;W)}{\epsilon}\leq \frac{H(W)}{\epsilon}$ rounds, the agreement protocol achieves $\epsilon$-MI consensus. 





\end{proof}

\yk{stop here}
